Asymptotic behaviour of large-scale solutions of Hitchin's equations in higher rank

Let $X$ be a compact Riemann surface. Let $(E,\theta)$ be a stable Higgs bundle of degree $0$ on $X$. Let $h_{\det(E)}$ denote a flat metric of the determinant bundle $\det(E)$. For any $t>0$, there exists a unique harmonic metric $h_t$ of $(E,\theta)$ such that $\det(h_t)=h_{\det(E)}$. We prove that if the Higgs bundle is induced by a line bundle on the normalization of the spectral curve, then the sequence $h_t$ is convergent to the naturally defined decoupled harmonic metric at the speed of the exponential order. We also obtain a uniform convergence for such a family of Higgs bundles.

==> new_theorem.tex <==
%newcounter
%\newcounter{goodsection}

%newtheorem
\newtheorem{thm}{Theorem}[section]
%\newtheorem{thmn}{$BDjM}(B}
\newtheorem{cor}[thm]{Corollary}
%\newtheorem{conj}[thm]{Conjecture}
\newtheorem{rem}[thm]{Remark}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{df}[thm]{Definition}
%\newtheorem{prob}[thm]{Problem}
\newtheorem{example}[thm]{Example}
\newtheorem{condition}[thm]{Condition}
\newtheorem{assumption}[thm]{Assumption}
%\newtheorem{principle}[thm]{Principle}
%\newtheorem{notation}[thm]{Notation}
%\newtheorem{convention}[thm]{Convention}
%\newtheorem{strategy}[thm]{Strategy}

